Active Learning with Partial Feedback

While many active learning papers assume that the learner can simply ask for a label and receive it, real annotation often presents a mismatch between the form of a label (say, one among many classes), and the form of an annotation (typically yes/no binary feedback). To annotate examples corpora for multiclass classification, we might need to ask multiple yes/no questions, exploiting a label hierarchy if one is available. To address this more realistic setting, we propose active learning with partial feedback (ALPF), where the learner must actively choose both which example to label and which binary question to ask. At each step, the learner selects an example, asking if it belongs to a chosen (possibly composite) class. Each answer eliminates some classes, leaving the learner with a partial label. The learner may then either ask more questions about the same example (until an exact label is uncovered) or move on immediately, leaving the first example partially labeled. Active learning with partial labels requires (i) a sampling strategy to choose (example, class) pairs, and (ii) learning from partial labels between rounds. Experiments on Tiny ImageNet demonstrate that our most effective method improves 26% (relative) in top-1 classification accuracy compared to i.i.d. baselines and standard active learners given 30% of the annotation budget that would be required (naively) to annotate the dataset. Moreover, ALPF-learners fully annotate TinyImageNet at 42% lower cost. Surprisingly, we observe that accounting for per-example annotation costs can alter the conventional wisdom that active learners should solicit labels for hard examples.

==> sections/contributions.tex <==
\paragraph{Contributions}
This key contributions of this paper are:
\begin{enumerate}
\item Introducing \emph{\problong{}}. 
\item Validating a deep learning method for learning from partial labels. 
\item Developing several sampling strategies for (example, concept pairs). 
\item We demonstrate superior accuracy under fixed budgets
and a considerable cost savings for annotation.
% \item \zack{We demonstrate that (our algorithm) fully annotates the dataset with just XXXk queries, compared to XXXk for the baseline model.}
\end{enumerate}

==> sections/discussion.tex <==
Traditional active learners treat human annotation as a black box. Because of this, human annotators often overwork for complicated labeling tasks and end up spending time less efficiently. Inspired by {\it Twenty Questions}, we develop an active learning framework that breaks down complicated labeling into natural binary questions, allowing annotators to provide partial feedback instead of full feedback. By doing so, annotators can focus on answering individual binary questions while learners are responsible for selecting the most valuable question and piecing together partial feedbacks. We experiment active learning with partial feedback on large-scale classification benchmarks. We find the proposed active learner achieves maximum performance and fully labels the data with 42\% less binary questions, comparing to passive learners and traditional active learners. Our diagnostic analysis suggests that it is more efficient to start active learning with ``easier'' data that can be cheaply annotated than with ``harder" data as often suggested by traditional active learning.

{\bf Future work:} We hope to expand our active learning with partial feedback framework onto multi-label classification, in which one annotators may assign multiple labels to each data. Another direction is to do real-world experiments and record the real annotation cost for different algorithms.

% \begin{itemize}
% \item Talk about how partial feedback is abundant in the real world. Users provide mark things as incorrectly labeled (without providing correct label) all the time.
% \item Experts, amateurs, and specialists.
% \item C
% \end{itemize}


==> sections/outline.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Justify the loss function,
%  and its effectiveness for deep modesl
%  
%  simple experiment: 
%  supervised (NOT ACTIVE)
%     for each example w prob p, assign 
%         y_i = exact label
%     w prob 1-p
%         label is a concept on path
%         from root to node, 
%         with each intermediate concept 
%         selected with equal probability
%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{DEVA MEETING TODO}
Big experimental todos. Determine (i) the effect of head start / seed set. (ii) what happens when difficulty is associated with.
\begin{itemize}
	\item EIG + $5\%$, $10\%$ partial feedback
	\item Add expected reduction in classes results
    \item Easy class attack on ERC. Save conversation for Discussion. 
    \begin{itemize}
    	\item EXPERIMENT: Take one class set it white.
        \item EXPERIMENT: Take two classes set white \& black.
        \item EXPERIMENT: More plausible: Make every dog the same dog dog. 
        \item EXPERIMENT: Dominant class / skewed dataset. Simplest case 1 class is 50\% of data. 
    \end{itemize}
    \item EASY: Represent Quantitative results in a table.
    \item Remove redundant from figure 7 (annotation)
   \item Plot that shows for a given method:
   what percentage of queries are at each level of the hierarchy. 
   \item Visualize the TRUE label distribution)\ of the SELECTED samples.
\end{itemize}

%
%   ZACK: Discussion WRITING TODOS
%
%   Draw connections to curriculum learning
%	Investigate pathological case
%
%	(or maybe in Experiments)
%	Discussissue of retraining from scratch
%	Mention that we tried pretraining and did worse.
%	MAKE POINT THAT PARTIAL FEEDBACK IS GENERALLY VERY IMPORTANT
%	Experts and amateurs, some might only be qualified to answer abstract question, others may only be specialists in a branch of the tree.
%
%    PEIYUN: see the paragraph Re-training in the Method section
%
%   Future Work
%   	Discuss how straightforward or not 
%   	it might be to generalize to case
%		where nodes in hierarchy have multiple 
%        / varying # of children
%		
%

\section*{\todo{Todos / Critical Points to Aniticipate}}
\begin{itemize}
\item Create a consistent glossary of terms.
\item Remove redundant plots (active data*) from annotation figure
\item \textbf{Anticipate criticism: that when class E is much easier than $k-1$ other classes, ERC may focus exclusively on class E until running out of examples. The easy ones have almost 100\% confidence, so always have minimum: 1 expected remaining class.}
\begin{itemize}
	\item Take tiny imagenet. 
    \item Pick $C$ classes (maybe 1? maybe 4?). 
    \item Make them artificially easy. 
    \item if one class, make all white
    \item if 4 classes, put a big white block in corresponding quadrant. 
    \item does ERC get distracted and pick only examples belonging to those $C$ classes???
    \item This compromises ERC in active learning setting, but not in data annotation setting. \textbf{Key difference:} in data annotation, must query every example at least once. 
\end{itemize}
\item in annotation plot (currently Fig 7), EIG has a staggering come from behind gain. The slope towards the end of annotation is better than for ERC
\begin{itemize}
	\item What happens if we have $500$k examples? 1M
    \item Even by accuracy -- EIG starts slower than EVERYTHING, then has a fast catchup.
    \item It's common in active learning (especially w deep nets) to start each model with a subset of labeled data. 
    \item How does that change things? Does that ameliorate EIG's early disadvantage?
\end{itemize}
\item Make a figure that shows the average number of partial labels the selected questions lead to (when answered with a yes)
\item Make a figure that shows the average reduction in the remaining classes (not the expected outcome). 
\item 
\end{itemize}

